A New Doctrine for Hardware Security

In this paper, we promote the idea that recent woes in hardware security are not because of a lack of technical solutions but rather because market forces and incentives prevent those with the ability to fix problems from doing so. At the root of the problem is the fact that hardware security comes at a cost; Present issues in hardware security can be seen as the result of the players in the game of hardware security finding ways of avoiding paying this cost. We formulate this idea into a doctrine of security, namely the Doctrine of Shared Burdens. Three cases studies---Rowhammer, Spectre, and Meltdown---are interpreted though the lens of this doctrine. Our doctrine illuminates why these problems and exist and what can be done about them.

==> Makefile <==
PAPER	= main
TEX	= $(wildcard *.tex)
BIB	= $(PAPER).bib
FIG	= $(wildcard figures/*.*)
LATEX	= pdflatex -shell-escape
BIBTEX	= bibtex
TITLE = title
OUTPUT = submission

.PHONY: all clean join spellcheck

all: $(PAPER).pdf

$(PAPER).bbl: $(BIB)
	$(LATEX)	$(PAPER)
	$(BIBTEX)	$(PAPER)

$(PAPER).pdf: $(PAPER).bbl $(TEX) $(FIG)
	$(LATEX)	$(PAPER)
	$(LATEX)	$(PAPER)

join: $(PAPER).pdf
	$(LATEX) $(TITLE)
	pdftk $(TITLE).pdf $(PAPER).pdf output $(OUTPUT).pdf
	rm $(TITLE).pdf

clean:
	$(RM) *.aux *.bbl *.blg *.log *.out $(PAPER).pdf

spellcheck:
	for i in *.tex; do \
    	aspell -c -t $$i ; \
	done

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> architectures.tex <==
\section{Architecting Systems to Implement a Doctrine of Shared Burdens} \label{sec:architectures}

The current generation of hardware vulnerabilities foreshadow a
grim future in which these vulnerabilities become the norm rather than the exception. 
% This is due to increasing product complexities from increased integration and excessive optimizations to simultaneously harvest the benefits of Moore's Law advances and at the compensate for slowdowns in Dennard scaling, and meet consumer expectations.
Trends of increased system integration and increased product complexity, enabled by Moore's law and propelled by consumer expectations, promise that more vulnerabilities are yet to be introduced and discovered.
This suggests that it would be advantageous to build our doctrine into our systems rather than only using it once the vulnerabilities are discovered.  
In this section we suggest how future systems could be architected to better implement a doctrine of shared burdens.

\subsection{Architectures for Swift Justice}

Consider the scenario where a Vendor discovers a patchable hardware vulnerability in their product. 
The Vendor begins taking the necessary steps to patch the problem, but discovers that the patch will cause a significant hit to performance when pushed to customers. 
% In this scenario, it is in the Vendor's rational interest to 
If the vulnerability was externally discovered, a Vendor may rationally decide to delay the patch release until the end of the disclosure embargo period, and may even extend the embargo period in an attempt to forestall the patch and its performance penalties and the subsequent loss of competitiveness in the marketplace.
If the vulnerability was internally discovered, a rational Vendor may not even disclose the vulnerability at all.
% a) delay the patch release to the end of the embargo period (if the vulnerability was reported by an external entity), or potentially not disclose the vulnerability at all if it was internally discovered, and 
% b) if the issue was reported by an external party, the Vendor can potentially keep requesting extensions to the embargo period.  
% This strategy is advantageous to Vendors in cases where the patch lowers performance of the Vendor's product compared to the competitors. 
Both cases, instigated by the Vendor's rational self-interest, are to the detriment of security overall. 
What can we do to prevent this scenario from happening?
What can we do to force the Vendor to
enhance security in a timely manner when there is a performance
cost?

The current paradigm is that if a Vendor releases a performance-sapping patch that it the burden of the Users to accept this cost as part of owning technology.
But according to our Doctrine of Shared
Burdens, this scenario should be interpreted as the Vendor offloading the cost of
an insecure and flawed design onto the User. 
In economic terms, the Vendors is externalizing the cost of their own insecurity.
We see this as an injustice facing Users today.

Current non-technical fixes to this problem are largely unsatisfactory.
Users could invoke the legal power of an Authority in a class action
lawsuit to correct this problem.  While this mechanism \textit{could}
motivate the Vendors to improve the security of their products, it
is not timely or efficient enough to be considered justice: There
is little if not no precedent of such class action lawsuits in the
realm of computer hardware, and legal battles would be protracted
and expensive.  Meanwhile, all users of the defective product are
continuously paying for the cost of insecurity in the form of the
performance-sapping patch.  The lack of swift action denies justice
to the Users.  As the maxim goes, justice delayed is justice denied.

To enable swift justice, we envision and present the use of
performance-security contracts that can be automatically settled between
Vendor and User without the explicit intervention of the Authority. 
The scheme would work as follows: 

\begin{enumerate}

\item Authorities would require all Vendors to provide
performance-security contracts to users. 

\item Authorities would require all internal and external
vulnerabilities to be registered with the Authority as soon as they
become known to the Vendors. Non-compliance will lead to stiff penalties
(including license to operate) as working rules of the Authorities.

\item Authorities will start monitoring the development
of patches for the vulnerability.  As soon as the patches are
available they are pushed out to the users.

\item Once the patches are deployed, the Users' hardware
starts monitoring the performance drop seen by the user based
on the patch.  
Note that the performance loss will be different per User and highly dependent on User workloads.
% Note that different users may encounter different performance drops based on their work patterns.

\item A rebate or credit will be given to the Users based on the measured performance loss.
% Based on the measured performance drop an agreed
% upon rebate or credit will be given to the users.  
This rebate/credit
can be converted to real money if desired based on conversion rates
set by the Authorities, a function that can be performed by experts
who price products based on what users value most.

\end{enumerate}

The above scheme is fair and equitable to Users and Vendors, and
enhances the state of security in a timely manner: If a User does
not turn on the computer, or does not use workloads that are impacted
by the fix, then the Vendor does not have to provide credits.  If
the Vendors delay patches, then Authorities can impose penalties.
The inclusion of Vendors in the Authorities (along with Consumer
Advocates) ensures that Authorities do not abuse their power. 

To enable proper implementation, and checks and balances in the
above system, a number of technical challenges have to be resolved.

\begin{enumerate}[listparindent=1.5em]

\item Computer hardware designers need to determine how
to measure the overhead of defense.  This raises two questions:
What is the overhead?  And, how exactly should it be measured?
There are number of options of answering the first question: energy, performance,
responsiveness, or even user frustration as measured by a camera \cite{grafsgaard2013automatically},  or some combination thereof based on the market
segment.  The infrastructure necessary for these measurements is
more or less available in most systems.  The second question is
likely more challenging, as it requires us to estimate the overhead 
of the defense without running
the insecure version of the system.  This estimation can be based
on mechanistic models of hardware, or based on data-driven models
trained on a large number of cases run with and without the
defense.
%  but essentially would require very accurate performance prediction.

\item Once a suitable measurement framework is determined,
computer architects need to find ways to ensure the integrity
of the reported data; Otherwise, a malicious User could alter or
fabricate the cost of defense in hopes of a higher credits from the
Vendor.  We expect that cryptography and tamper-resistant hardware
will play a role in achieving this constraint.

\item There is also a need to continuously audit the
defenses themselves.  Once a hardware vendor pushes out a defense,
how do the Authorities and Users know that the Vendor's final product
actually implements the defense in a satisfactory manner?  How do
we know that a Vendor has actually taken on the burden of
defense, and hasn't instead forgone the defense in favor of higher
run time performance?
Or if the Vendor uses an adaptive,
best-effort strategy to implement a defense, how do we know that
the best-effort sufficiently deters attackers?  Likewise, how
do we know that Users have not turned off their defenses to gain
higher performance?

One might question if these concerns are realistic or warranted.
% We argue that one needs only to look to the automotive industry
Indeed, one needs only to look to the automotive industry for a recent example of how systems can be engineered to cheat audits.
In 2015, it was
revealed that Volkswagen automobiles were knowingly falsifying their
self-reported exhaust emissions levels.  By lying about emissions
levels, Volkswagen's automobiles could achieve a better fuel
efficiency while still appearing to conform to exhaust emissions
regulations, thus giving Volkswagen a competitive edge in the
marketplace.
If we intend to audit the presence of security, we must anticipate that Vendors (and Users) will try to do the same.

We suggest building auditing support in hardware to mitigate this
concern.
Periodically, the Authorities would run attacks on hardware
to determine if the defenses are working as provisioned.  The
hardware must be designed in a way that executing the (test) attack
does not interfere with the normal performance of the hardware to
avoid ethical issues.  Design of such auditing mechanism requires
test lanes, test memory, etc.,  to be reserved in the hardware for the attacks.  Minimizing the cost of such infrastructure is a significant challenge.

\end{enumerate}

\subsection{Punitive Architectures} We should expect cybercrime to
continue for as long as the criminals are able to act with near
impunity \cite{anderson2019measuring}.  
This dynamic is unlikely to change anytime soon, as there is currently no notion
of a ``punitive'' architecture in computer hardware.  
We describe an architecture as punitive if it either 1) includes hardware support that will enable criminal attackers to be prosecuted by law
enforcement channels, or 2) deters attacks by delaying and preventing attackers from causing harm.

What is the use case for such a system?  Consider a cloud system.
If a VM is carrying out a microarchitectural attack on another
co-located instance, it would be valuable to log information on the
VM, the processes are running in both VMs, and the data
collected so it can be used for prosecution if such a need arises.
Of course, this seems unachievable without compromising privacy to
some degree.  
To address this, any loss of privacy due to implementing this solution
should first be disclosed in clear terms to the Users.  
Second, this level of privacy loss may not be as unprecedented as it may first appear, and may be more acceptable to Users than one might initially expect. 
For instance, companies usually monitor large amounts of internal traffic and
behavioral data to detect insider threats, analogous to security cameras in a building.
The privacy loss of such a scheme is likely comparable to such monitoring frameworks.

If evidence collection towards attribution is unachievable because of privacy concerns, we must think of other ways to design deterrence into our systems.  
If the attacker has specific signature
moves, it could be possible to isolate the attacker and move them to a different, quarantined machine.  
Going back to the cloud example, if one
instance is suspected to be attacking another co-located instance,
the attacker instance can be migrated to another machine where there
is no co-location~\cite{demme2013feasibility}.
This other machine needs to be a bit slower so the attacker does not use this strategy to get higher performance. 
%CITE John Demmes' ISCA 13 paper on AV, look at the last page

Another possible solution is to slow down parts of the computer that are used
more by Attackers than everyday Users. 
For instance, high precision clocks are rarely needed in normal programs yet are used very commonly in attacks. 
It should be possible to slow down these clocks intentionally to frustrate and delay attackers ~\cite{martin2012timewarp, kohlbrenner2016trusted}. 
We refer to these as asymmetrical defenses.

In our goal of asymmetrical defenses, we also see the need for smaller, 
faster, and more accurate anomaly detectors that
can identify the Attackers' behavior and frustrate their efforts.
To minimize the always-on cost of defense to the Users,
we need to design our defenses to be scalable so that
the full weight of defense is only applied to a system during periods
of highly suspicious behavior.  Only once these two goals are met
can our systems truly find the right balance between always-on
defenses (which burden the User) and adaptive defenses (which burden
the Attacker).  Such asymmetrical defenses should be a top design
priority in future hardware.


% \subsection{Open Source}

% How do recent trends towards open-source hardware fit into our doctrine?
% Open source may seem like thorn in the side of our doctrine---after all, how can you assign a ``burden'' of security to an open-source project with no 

% We can answer this by first looking at open source in the context of software, where the concept originated.
% % We will first talk about open source in the context of software, where the concept originated.
% Open source software is a controversial topic among security researchers.
% On one hand, open source software can be great for security, because anyone can inspect the source code, and as the saying goes, ``given enough eyeballs, all bugs are shallow'' (security bugs included).
% But on the other hand, 

% open source projects are available ``as-is'' and come with no warranty or security guarantees, 
% Open source software is typically available to use ``as-is'' and comes with no guarantees 
% Compounding this problem is that free and open source software isn't really owned by anyone, so how do we 
% % Open source HW

% Many of the security challenges of open source software come from the fact that software is a very abnormal product, as it has no physical components and is essentially free to reproduce and distribute.
% But open source \textit{hardware} is different.
% % It does cost something to make and distribute
% No one is going to do it for free
% So even though you may have open source HW, at the end of the day someone is going to be selling you a physical thing.
% Then consumer protection laws should apply.
% If a hardware vendor is using open source, they should be held liable for the security of their product
% So they shouldn't be able to use ``open source'' as an excuse to sell an insecure product.
% Should be up to them to decide if whatever open source is safe or not.




==> nontech.tex <==
\section{Non-Technical Issues} \label{sec:nontech}

A holistic approach to our Doctrine of Shared Burdens requires more
than just technical solutions  to improve security. 
In this section, we outline some non-technical measures
may be needed as well.

As a first example, we point out  that our technical solution (architectures for swift justice) does
not offer explicit incentives to solve the prisoner's dilemma towards
solving security problems.  
Specifically, our schemes do not offer any incentives for companies to be first movers towards making their systems more secure, especially when security comes at a cost to performance.
Non-technical solutions are needed for this problem.


To move the market, we suggest that the Authorities could introduce
a mandate that {\it requires a certain fraction of the advertised
insecure peak performance and/or operational energy to be set aside
for security measures.}
This mandate should be satisfied by all Vendors but gives individual
Vendors complete flexibility in implementing how this
set-aside should be used for security.  This type of mandate has
several advantages:
\begin{enumerate}[listparindent=1.5em]

\item It can help Vendors innovate in terms of
security without worrying what they will lose out in terms of
performance if their competitor spends less on security.  In a
manner of speaking this levels the playing field for security.

\item It is not prescriptive in telling the Vendors exactly which problems to fix, and allows Vendors to select specific solutions that demand attention based on their own estimate of risk and demand. 

\item It allows Vendors to address 0-day vulnerabilities on their own and removes the incentive to hide internally-discovered vulnerabilities, since any performance loss from patches can be ``absorbed'' by the set aside performance dedicated towards security.

% \item It creates an audit trail for Authorities to know about what features are considered by the Vendors as security features so they can be audited (using solutions described in the previous section).  In other words, it breaks down some barriers towards information asymmetry.

\item It identifies the features the Vendors consider to be security features and creates an audit trail for the Authorities to monitor (using solutions described in the previous section).  
In other words, it breaks down some barriers towards information asymmetry by disclosing how Vendors respond to threats.

\end{enumerate}

Another largely non-technical issue is the need for widespread security education among engineers.
Since a computer engineer's ineptitude can cause harm to a
User, it may be needed to require engineers to pass some kind of
licensing exam proving they are competent at secure design, similar
to the way a lawyer or medical doctor must pass exams administered
by an Authority before they are able to practice in their field.
Due to the ever-changing nature of security and threats, such a
licensing will likely need to be periodically renewed so that
engineers are up-to-date on the latest and best practices.


% Sec 2: Market Failures in Hardware security

% HW Security: Anything microarchitectural and that has an architectural difference

% Market Failures: How exactly these issues manifest in the context of hardware security. It's OK to be repetitive---just ✔

% Prisoner's Dilemma: Law enforcement (not judge) ✔

% 2.2 Unique Challenges: Each Para needs to have a starting boldface saying what the paragraph is about ✔
% (four item not three) ✔
% Sec 2: Motivation instead of Background ✔
% Doctrine of Shared/Joint Efforts
% Effort: something that's hard

% flawed: Too strong a word
% Sec 3: Shared Burdens---Attackers is much longer ✔
% So add to Vendors, Users, etc. ✔
% Say what they can do to implement the Doctrine ✔
% Authority might mandate Vendors use 2FA ✔
% Attackers---last para too detailed. Hint the reader ✔
% Make something relevant to hardware in each section ✔
% User should apply patches and not turn of security ✔

% Sec 4: Rename "Difference from prior Doctrines" ✔
% Prior doctrines: Focus on why they don't apply to hardware 
% Formal ISAs have been formally verified but not for side channels.
% Sel4: No KPTI
% Warren Hunt UT Austin formally verified OOO processor ✔
% Doctrine of Risk Management: Talk about why it doesn't work for Hw
% e.g. for MDS attacks, recommendation is to turn of hyperthreading but vendors have determined that the risk is not worth item
% Why DRM is not a good idea for HW: Hard to evaluate risk

% 4.3 Change to "Doctrine of Deterrence" ✔

% Public Goods: Why it doesn't work for HW (not generally)

% Case Studies: Too fluid. Take a stance (standards needed for security)

% DRAM: not clear how the defense is asymmetric. Bring together in crisp manner. What did rowhammer get right? ✔

% Same for who should fix Spectre. 
% Case Studies should teach something
% Prisoner's Dilemma nobody wants to make the first move ✔
% Intel saying it's the browser's job to fix the problem
% Turn off speculation when entering security-sensitive code 
% Puts burden on programmers who are unaware of spec execution 
% Principle of Least Concern

% Meltdown
% don't just talk about Intel vs AMD, because some ARM vulnerable as well.
% In the x86 world, it was only Intel
% Don't heat so much on Intel
% The market eventually fixed, but huge disclosure gap between when they knew and when it was announced. Intel knew early 2017
% Metaproblem is that there is a gap between when things are identified and when things are disclosed.
% Market did not work perfectly.
% Regulators still have a role
% Not just Meltdown
% Look at MDS that came later
% Even though recommended fix is disable hyperthreading, HW manufacturers have been reluncatnat to make that fix because they assess the risk to be low
% Google RIDL attack
% It's not for Intel to decide
% Should be Authority (SRO) to decide which vulns get fixed
% SRO should have practitioners. A third party to determine risk

% Two problems: Future problems (patching) and known problems 
% How to 
% Take out comment on note to Simha (domain bypass)

% Meltdown: Free market may appear to work but there's room for improvment 

% Rowhammer defense: Shifting burdens over time 
% Spectre: How does the Burden over time
% Meltdown: Same:

